Reducing Turbulence-Induced Outages in a Deployed Terrestrial Free-Space Optical Communication Link via Interleaving

We present an experimental study of data interleaving for terrestrial free-space optical communication over a 4.6~km urban testbed. Results demonstrate a two-order-of-magnitude reduction in outage probability. A dependency between measured turbulence strength, interleaver length, and achievable data rate is revealed, enabling robust system design.

==> tikz/Scint_Cn2_October.tex <==
  \begin{tikzpicture}[>=latex]
\begin{axis}[
every axis/.append style={font=\small},
tick label style={font=\footnotesize},
ylabel = $C_n^2$ (m$^{-2/3}$),
xlabel = Time,
xmin = 0, xmax =432,
ymin = 1e-16, ymax = 1e-14,
ymode = log,
xtick distance = 72,
xticklabels = {0,12.00,24.00,12.00,24.00,12.00,24.00,12.00},
x tick label style={yshift= -1mm},
y tick label style={xshift= -1mm},
ylabel shift = 1mm,
xlabel shift = 1mm,
set layers, mark layer=axis tick labels,
width = 11.3cm,
 height = 3.6cm,
 grid = major,
 xlabel near ticks,  
 ylabel near ticks,  
 xticklabel style={/pgf/number format/fixed},
every axis plot/.append style={thick},legend style={at={(0.05,0.3)},anchor=west, font = \scriptsize,row sep=-0.75ex,inner sep=0.2ex, fill opacity = 0.6, text opacity = 1},
legend cell align={left},
]

\pgfplotstableread{Figures/Scint_Cn2_October.txt}
\datatable
\addplot[C2, mark = none,thick,unbounded coords=jump]
             table
         [
          x expr=\thisrowno{0}, 
          y expr=\thisrowno{1} 
         ] {\datatable};
\draw[thick,dashed] (axis cs: 71,1e-16) -- (83,1e-14);
\draw[thick,dashed] (axis cs: 215,1e-16) -- (227,1e-14);
\draw[thick,dashed] (axis cs: 359,1e-16) -- (371,1e-14);

\node[align = center] at (axis cs: 45
,4e-15){Oct. 10$^{\text{th}}$ \\ 2025} ;
\node[align = center] at (axis cs: 184,4e-15){Oct. 11$^{\text{th}}$ \\ 2025};
\node[align = center] at (axis cs: 332,4e-15){Oct. 12$^{\text{th}}$ \\ 2025};
\node[align = center] at (axis cs: 395,4e-15){Oct. 13$^{\text{th}}$\\ 2025};

\draw[C0,->, very thick] (axis cs: 107,1.5e-15) -- (axis cs: 107, 2.2e-16);
\draw[C4,->, very thick] (axis cs: 143,8e-15) -- (axis cs: 143, 1.35e-15);
\draw[C3,->, very thick] (axis cs: 300,1.04e-15) -- (axis cs: 300, 6.8e-15);

\node at (axis cs: 419, 1.7e-16) {(b)};

\filldraw[black, opacity = 0.2] (axis cs:359,1e-14) rectangle (axis cs:370,1e-16);

\filldraw[black, opacity = 0.2] (axis cs:373,1e-14) rectangle (axis cs:376,1e-16);

\filldraw[black, opacity = 0.2] (axis cs:389,1e-14) rectangle (axis cs:422,1e-16);

\filldraw[black, opacity = 0.2] (axis cs:430,1e-14) rectangle (axis cs:431,1e-16);
\end{axis}
\end{tikzpicture}

==> tikz/Scint_Cn2_September.tex <==
  \begin{tikzpicture}[>=latex]
\begin{axis}[
every axis/.append style={font=\small},
tick label style={font=\footnotesize},
xlabel = $C_n^2$ (m$^{-2/3}$),
ylabel = Occurrences,
xmin = 6e-17, xmax =3e-14,
xmode = log,
ymin = 0, ymax = 200,
xtick distance = 150,
grid = minor,
xtick = {1e-16,1e-15,1e-14,1e-13},
x tick label style={yshift= -1mm},
y tick label style={xshift= -1mm},
ylabel shift = 1mm,
xlabel shift = 1mm,
set layers, mark layer=axis tick labels,
width = 11.3cm,
 height = 3.6cm,
 xlabel near ticks,  
 ylabel near ticks,  
 xticklabel style={/pgf/number format/fixed},
every axis plot/.append style={thick},legend style={at={(0.05,0.3)},anchor=west, font = \scriptsize,row sep=-0.75ex,inner sep=0.2ex, fill opacity = 0.6, text opacity = 1},
legend cell align={left},
]

\pgfplotstableread{Figures/Scint_Cn2_September.txt}
\datatable
\addplot[C2, mark = none, fill = C2!50, ybar interval]
             table
         [
          x expr=\thisrowno{0}, 
          y expr=\thisrowno{1} 
         ] {\datatable};
\draw[C0,fill = C0!90, thick] (axis cs: 2.13286e-16, 0) rectangle (axis cs: 2.42127e-16,103); 
\draw[C4,fill = C4!90, thick] (axis cs: 1.6227e-15, 0) rectangle (axis cs: 1.42948e-15,193); 
\draw[C3,fill = C3!90, thick] (axis cs: 6.54861e-15, 0) rectangle (axis cs: 7.43413e-15,87); 

\node at (axis cs: 2.5e-14,25) {(a)};

\node at (axis cs: 2.6e-16,170){Sept. 13$^{\text{th}}$ 2025 - Oct. 13$^\text{th}$ 2025};
\end{axis}
\end{tikzpicture}
